AutoReply: Detecting Nonsense in Dialogue Introspectively with Discriminative Replies

Existing approaches built separate classifiers to detect nonsense in dialogues. In this paper, we show that without external classifiers, dialogue models can detect errors in their own messages introspectively, by calculating the likelihood of replies that are indicative of poor messages. For example, if an agent believes its partner is likely to respond "I don't understand" to a candidate message, that message may not make sense, so an alternative message should be chosen. We evaluate our approach on a dataset from the game Diplomacy, which contains long dialogues richly grounded in the game state, on which existing models make many errors. We first show that hand-crafted replies can be effective for the task of detecting nonsense in applications as complex as Diplomacy. We then design AutoReply, an algorithm to search for such discriminative replies automatically, given a small number of annotated dialogue examples. We find that AutoReply-generated replies outperform handcrafted replies and perform on par with carefully fine-tuned large supervised models. Results also show that one single reply without much computation overheads can also detect dialogue nonsense reasonably well.

==> comments.tex <==
\begin{abstract}
    % so building strong diplomacy agents to communicate human is especially challenging. 
% As a first step towards competent diplomacy dialogue agent, we study the problem of how to detect nonsense in generated dialogues. 
% % Previous work has proposed to build supervised classification models. But since
% Given the multi-player multi-phase complex game setting, there are innumerable nonsensical situations in Diplomacy, and annotating them to build supervised classifiers is impractical. 
% In this paper, we propose to detect nonsensical messages under a few-shot learning setting with prompt-based learning. 
% The assumption is that certain follow-up replies like \emph{``i don't understand''} will have higher probabilities after a nonsensical message than after a reasonable message, and thus can be used to differentiate good and bad messages. %if the message is nonsensical, the probability of a follow-up reply like ``i don't understand'' will be higher than the case when the message makes sense, and thus discriminative. 
% We propose \ModelName, a contrasitive search algorithm to automatically generate discriminative follow-up reply prompt for the nonsense detection. 
% Experiments suggest that \ModelName can produce large amounts of discriminative follow-up replies and achieve significantly better nonsense detection results than hand-crafted replies. % such a few-shot approach is effective in nonsense detection and 

% Despite the progress in large-scale pretrained language models, these models are still making nonsense in dialogue generation. This problem  can be especially severe for dialogue applications in high-intellengent domains such as negotion and persuasions. but annotating all the nonsense messages can be costly and impractical for diplomacy because the situations are enumerous. Therefore, we propose to detect nonsense in an unsupervised fashion. by calculating the probability of follow-up responses like ``i don't understand''. 




% Diplomacy has been a long-standing benchmark game in AI research due to its huge action space and complex verbal communication dynamics. 
% Existing dialogue models still easily generate nonsensical messages, so building strong diplomacy agents to communicate human is especially challenging. 
% As a first step towards competent diplomacy dialogue agent, we study the problem of how to detect nonsense in generated dialogues. 
% % Previous work has proposed to build supervised classification models. But since
% Given the multi-player multi-phase complex game setting, there are innumerable nonsensical situations in Diplomacy, and annotating them to build supervised classifiers is impractical. 
% In this paper, we propose to detect nonsensical messages under a few-shot learning setting with prompt-based learning. 
% The assumption is that certain follow-up replies like \emph{``i don't understand''} will have higher probabilities after a nonsensical message than after a reasonable message, and thus can be used to differentiate good and bad messages. %if the message is nonsensical, the probability of a follow-up reply like ``i don't understand'' will be higher than the case when the message makes sense, and thus discriminative. 
% We propose \ModelName, a contrasitive search algorithm to automatically generate discriminative follow-up reply prompt for the nonsense detection. 
% Experiments suggest that \ModelName can produce large amounts of discriminative follow-up replies and achieve significantly better nonsense detection results than hand-crafted replies. % such a few-shot approach is effective in nonsense detection and 

% Despite the progress in large-scale pretrained language models, these models are still making nonsense in dialogue generation. This problem  can be especially severe for dialogue applications in high-intellengent domains such as negotion and persuasions. but annotating all the nonsense messages can be costly and impractical for diplomacy because the situations are enumerous. Therefore, we propose to detect nonsense in an unsupervised fashion. by calculating the probability of follow-up responses like ``i don't understand''. 

\end{abstract}

==> tables.tex <==
\begin{table*}[!htbp]
\centering
\begin{adjustbox}{width=0.95\textwidth}
\begin{tabular}{l|l|l|l|cccc|cccc|cccc}
\toprule
\textbf{Model(train: 4149/561, test: 1036/139)} &num prompts& coverage &n clf& \multicolumn{4}{c|}{\textbf{Train}} & \multicolumn{4}{c}{\textbf{Validation}}  & \multicolumn{4}{c}{\textbf{Test}} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
%\midrule
 &&&&  \textbf{Auc}&  \textbf{Prec} & \textbf{Recall} & \textbf{F1} &  \textbf{Auc}& \textbf{Prec} & \textbf{Recall}&\textbf{F1}&  \textbf{Auc}&  \textbf{Prec} & \textbf{Recall} & \textbf{F1}  \\
\midrule
"generated prompts higher recall 5 5"&16587&"(557, 561)"&250&65.73&32.58&43.67&37.32&60.34&27.50&31.88&29.53&65.15&31.58&42.86&36.36\\ 

"generated prompts higher recall 6 6"&10479&"(557, 561)"&190&64.57&33.33&39.93&36.33&60.29&29.17&30.44&29.79&64.40&32.56&40.00&35.90\\ 

"generated prompts higher recall 7 7"&6700&"(557, 561)"&118&66.46&32.45&45.81&37.99&61.84&27.78&36.23&31.45&66.43&30.84&47.14&37.29\\ 

"generated prompts higher recall 8 8"&6700&"(558, 561)"&118&66.46&32.45&45.81&37.99&61.84&27.78&36.23&31.45&66.43&30.84&47.14&37.29\\ 

"generated prompts higher recall 9 9"&2805&"(545, 561)"&51&67.00&30.27&49.38&37.53&63.58&27.36&42.03&33.14&67.12&28.80&51.43&36.92\\ 

"generated prompts higher recall 10 10"&1830&"(543, 561)"&32&67.36&28.60&52.41&37.00&63.68&25.41&44.93&32.46&67.82&27.27&55.71&36.62\\ 

"generated prompts higher recall 11 11"&1192&"(524, 560)"&27&65.08&31.22&42.96&36.16&58.94&24.42&30.44&27.10&64.85&27.83&45.71&34.59\\ 

"generated prompts higher recall 12 12"&790&"(507, 560)"&20&64.11&30.69&40.64&34.97&59.33&25.61&30.44&27.82&63.80&27.52&42.86&33.52\\ 

"generated prompts higher recall 13 13"&515&"(479, 559)"&12&64.95&28.48&45.28&34.96&58.46&21.30&33.33&25.99&65.31&26.77&48.57&34.52\\ 

"generated prompts higher recall 14 14"&322&"(445, 558)"&2&63.34&16.66&82.53&27.72&59.01&14.75&78.26&24.83&67.66&17.91&92.86&30.02\\ 

"generated prompts higher recall 15 15"&197&"(392, 554)"&2&65.14&18.63&73.98&29.76&56.50&14.48&60.87&23.40&67.24&19.64&77.14&31.30\\ 

"generated prompts higher recall 16 16"&197&"(401, 554)"&2&65.14&18.63&73.98&29.76&56.50&14.48&60.87&23.40&67.24&19.64&77.14&31.30\\ 

"generated prompts higher recall 17 17"&89&"(343, 552)"&2&65.14&20.85&62.21&31.23&55.86&15.00&47.83&22.84&66.35&21.20&65.71&32.06\\ 

"generated prompts higher recall 18 18"&56&"(302, 551)"&1&62.65&16.98&74.69&27.67&54.62&13.52&62.32&22.22&62.18&16.61&75.71&27.25\\ 

"generated prompts higher recall 19 19"&36&"(259, 550)"&1&62.19&17.66&65.95&27.86&53.69&13.43&52.17&21.37&64.90&18.61&72.86&29.65\\ 

"generated prompts higher recall 20 20"&18&"(181, 513)"&1&60.35&17.67&55.97&26.86&49.83&11.66&37.68&17.81&63.96&19.56&62.86&29.83\\ 

"generated prompts higher recall 21 21"&14&"(154, 504)"&1&59.03&17.45&50.09&25.89&48.23&10.66&30.44&15.79&63.36&19.90&58.57&29.71\\ 

"generated prompts higher recall 22 22"&11&"(153, 498)"&1&58.93&17.48&49.38&25.81&48.62&10.88&30.44&16.03&63.55&20.10&58.57&29.93\\ 

"generated prompts higher recall 23 23"&5&"(85, 362)"&1&56.96&21.99&26.74&24.14&51.79&14.67&15.94&15.28&59.38&23.96&32.86&27.71\\ 

"generated prompts higher recall 24 24"&4&"(76, 301)"&1&56.47&21.68&25.31&23.36&52.08&15.28&15.94&15.60&59.05&24.18&31.43&27.33\\ 

"generated prompts higher recall 25 25"&3&"(69, 271)"&1&56.22&22.00&23.89&22.91&51.45&14.29&14.49&14.39&59.34&25.00&31.43&27.85\\ 

"generated prompts higher recall 26 26"&3&"(72, 271)"&1&56.22&22.00&23.89&22.91&51.45&14.29&14.49&14.39&59.34&25.00&31.43&27.85\\ 


\bottomrule
\end{tabular}
\end{adjustbox}
\caption{use classifiers of different recalls}
\label{tab:main}
\end{table*}







\begin{table*}[!htbp]
\centering
\begin{adjustbox}{width=0.95\textwidth}
\begin{tabular}{l|l|l|l|cccc|cccc|cccc}
\toprule
\textbf{Model(train: 4149/561, test: 1036/139)} &num prompts& coverage &n clf& \multicolumn{4}{c|}{\textbf{Train}} & \multicolumn{4}{c}{\textbf{Validation}}  & \multicolumn{4}{c}{\textbf{Test}} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
%\midrule
 &&&&  \textbf{Auc}&  \textbf{Prec} & \textbf{Recall} & \textbf{F1} &  \textbf{Auc}& \textbf{Prec} & \textbf{Recall}&\textbf{F1}&  \textbf{Auc}&  \textbf{Prec} & \textbf{Recall} & \textbf{F1}  \\
\toprule


%Supervised Learning (no SL, because the contrastive examples are generated) &-&&  &  &  &  & &  \\% 

% Paraphrased Manual Prompts(???) &- && \textbf{93.93} & 91.72 & 96.25** & 20.60 & 26.65 & 16.96 \\% 

%No Manual Prompts (setting threshold) &-&&  &  &  &  & &   \\% 

"subset justification 9"&2805&"(40, 561)"&51&74.81&1.25&92.50&2.47&56.85&1.86&100.00&3.65&77.77&2.82&100.00&5.49\\ 

"justification None"&5486&"(39, 30)"&913&68.13&1.96&70.00&3.82&71.04&3.19&71.43&6.10&70.05&4.52&72.73&8.51\\ 

\midrule
"subset justification fewshot 9"&2805&"(40, 561)"&51&72.31&0.17&100.00&0.34&56.85&1.86&100.00&3.65&77.77&2.82&100.00&5.49\\ 

"justification few shot None"&9673&"(5, 5)"&999&55.37&0.14&100.00&0.27&55.60&1.50&100.00&2.95&55.50&2.33&100.00&4.55\\ 

\bottomrule






% \midrule
% Majority vote&-&&  &  &  &  & &   \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{wrong justification classification result (for categories that we don't know how to design manual prompts)
 }
\label{tab:invalid order}
\end{table*}



\begin{table*}[!htbp]
\centering
\begin{adjustbox}{width=0.95\textwidth}
\begin{tabular}{l|l|cccc|cccc|cccc}
\toprule
\textbf{Model} &\textbf{num}& %coverage &n clf&
\multicolumn{4}{c|}{\textbf{Train}} & \multicolumn{4}{c|}{\textbf{Validation}}  & \multicolumn{4}{c}{\textbf{Test}} \\ 
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
%\midrule
 &&  \textbf{Auc}&  \textbf{Prec} & \textbf{Recall} & \textbf{F1} &  \textbf{Auc}& \textbf{Prec} & \textbf{Recall}&\textbf{F1}&  \textbf{Auc}&  \textbf{Prec} & \textbf{Recall} & \textbf{F1}  \\
\midrule


Supervised Learning &-&&  &  &  & &  & \\% 
% \midrule


Hand-crafted best&14&%"(nan, nan)"&10&
60.05&22.41&37.79&28.13&59.81&22.52&36.23&27.78&58.73&20.31&37.14&26.26\\ 

% Hand-crafted all&47&%"(nan, nan)"&25&
% 57.83&14.34&81.46&24.39&59.36&14.46&88.41&24.85&60.37&15.06&87.14&25.68\\ 
% \midrule
Model-generated &8834&%"(nan, nan)"&5&
\textbf{93.84}&\textbf{99.80}&\textbf{87.70}&\textbf{93.36}&58.94&24.42&30.44&27.10&59.05&24.18&31.43&27.33\\ 
\midrule
DipPK (recall=21/561) &14&%"(154, 504)"&1&
59.03&17.45&50.09*&25.89&48.23&10.66&30.44&15.79&63.36&19.90&\textbf{58.57*}&29.71\\ 

% DipPK (recall=19/561) &36&%"(259, 550)"&1&
% 62.19&17.66&65.95&27.86&53.69&13.43&52.17&21.37&64.90&18.61&72.86&29.65\\ 
% \midrule

% "complete separate None"&8593&"(312, 442)"&52&57.02&14.88&62.03&24.00&55.39&13.99&59.42&22.65&57.10&14.87&62.86&24.04\\ 

% "complete separate manual picked None"&202&"(23, 56)"&1&52.97&15.99&20.50&17.97&51.65&14.12&17.39&15.58&50.83&12.84&20.00&15.64\\ 
% \midrule

% "generated prompts higher recall 7 7"&6700&"(557, 561)"&118&66.46&32.45&45.81&37.99&61.84&27.78&36.23&31.45&66.43&30.84&47.14&37.29\\ 

% "generated prompts higher recall manual picked 7 7"&199&"(361, 560)"&1&61.98&16.47&76.29&27.09&62.10&15.95&81.16&26.67&61.83&16.31&77.14&26.93\\ 
% \midrule

DipPK (recall=9/561) &2805&%"(545, 561)"&51&
67.00*&30.27*&49.38*&37.53*&\textbf{63.58}&\textbf{27.36}&42.03&\textbf{33.14}&\textbf{67.12*}&\textbf{28.80*}&51.43*&\textbf{36.92*}\\ 

DipPK (recall=9/561), picked&82&%"(257, 554)"&1&
61.63&18.49&57.58*&27.99&60.89&17.00&\textbf{62.32*}&26.71&57.63&16.28&50.00*&24.56\\ 
% \midrule

% "both separate and generated 9 9"&11398&"(550, 561)"&119&65.81&21.09&63.99&31.73&59.92&17.45&53.62&26.33&67.22&22.12&65.71&33.09\\ 


% \midrule
% Majority vote&-&-& 0 & 0 & 0 &0  &0 &0   \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Main  classification result from the model ensemble. \textbf{num} is the number of replies in the ensemble. We perform t-test against ``hand-crafted best''.}
\label{tab:main}
\end{table*}






% supervised learning vs autoreply


\begin{table*}[!htbp]
\centering
\begin{adjustbox}{width=0.95\textwidth}
\begin{tabular}{llrrrrrrrr}
\toprule
 && %coverage &n clf&
% \multicolumn{4}{c}{\textbf{Train}} & 
\multicolumn{4}{c}{\textbf{Validation}}  & 
\multicolumn{4}{c}{\textbf{Test}} 
\\ 
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
% \cmidrule(lr){11-14}
%\midrule
 \textbf{Training Data} & \textbf{Model} &  
%  \textbf{Auc}&  \textbf{Prec} & \textbf{Recall} & \textbf{F1} &  
 \textbf{Auc}& \textbf{Prec} & \textbf{Recall}&\textbf{F1}&  
 \textbf{Auc}&  \textbf{Prec} & \textbf{Recall} & \textbf{F1}  
 \\
\midrule




 %(recall$\geq$9/561) 
\multirow{2}{30mm}{$B$+$G$, 561+561}&\ModelName (num=2805)&%"(545, 561)"&51&
% 67.00\rlap{$^*$}&30.27\rlap{$^*$}&49.38\rlap{$^*$}&37.53\rlap{$^*$}&
63.58&27.36&42.03&33.14&
67.12&28.80&51.43&36.92\\ 


 & Supervised Learning & 
% 80.12 & 81.41 & 78.07 & 79.71 &
70.06 & 24.47 & 68.12\rlap{$^*$} & 36.02 &
71.85  &25.24 &  72.86\rlap{$^*$} &37.50 \\% 
\midrule
% 50

 %(recall=30)
\multirow{2}{30mm}{$B$+$G_{50}$, 561+50} & \ModelName (ng=50) &

% 58.26&22.22&31.37&26.02&
63.53&32.10\rlap{$^*$}&37.68&34.67\rlap{$^*$}&
56.99&20.19&30.00&24.14\\ 


 %(recall=30)
& Supervised learning (ng=50) & 

% 58.26&22.22&31.37&26.02&
58.47&15.98&56.52\rlap{$^*$}&24.92&
65.35\rlap{$^*$}&19.16&71.43\rlap{$^*$}&30.21\\ 
\midrule

% invalid orders
 %(recall$\geq$4/79)
\multirow{2}{30mm}{Invalid Order subset from $B$+$G$, 79+561} &\ModelName (num=1609, order)&
% 58.16&19.44*&17.72&18.54&
55.46&50.00&11.11&18.18&
60.23&37.50&21.43&27.27\\ 





  &Supervised Learning & 
% 87.70  & 50.74  & 87.34  & 64.19  &
64.79  & 4.94  & 44.44\rlap{$^*$} & 8.89 &
74.42\rlap{$^*$} & 10.11 & 64.29\rlap{$^*$} & 17.48\\% 



\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
% Main  classification result from the model ensemble. \textbf{num} is the number of replies in the ensemble. We perform t-test against ``Hand-crafted''. ``\ModelName (num=$x$)'' is the subset of \ModelName-generated replies of size $x$. 
%  ``\ModelName (num=2805)'' achieves significantly better classification results than all the baselines. ``\ModelName (num=14)'' contains only 14 replies, and is still better than the baselines, suggesting the generated replies are of high-quality. ``\ModelName (num=2805, picked)'' is a subset of ``\ModelName (num=2805)'' selected using human-defined keywords like ``can't'', suggesting that integrating human knowledge doesn't work.
 }
\label{tab:sl}
\end{table*}



%%%%%%%%%%% coverage
\subsubsection{Coverage}
\label{sec: coverage}
% We also want to know how many bad message examples the \ModelName-generated replies can detect. 
One intuition is that the more replies we have, the more bad examples we can cover, and thus the better the classification is. So we calculate the coverage, the number of bad training examples that can be correctly detected by the union of the \ModelName-generated replies 
% the size of the union of the bad training examples each \ModelName-generated reply can correctly predict as nonsense,
$|\cup_r \{B_i|\log P_{B_i}(r)>t_r\}|$, to see its impacts.  
Figure~\ref{fig:coverage} shows the coverage and test F1. 
As we increase the recall, at the beginning, the coverage stays the same, and the test F1 increases as the recall get higher; but as we further increase the recall, there will be fewer and fewer reply prompts, and the coverage  decreases, and the test F1 also drops. This verifies our intuition to some extend and shows that coverage is correlated with the classification. If the coverage is not impacted, we can improve the F1 by choosing the subset with higher recalls. % reduce the prompts and. Coverage means how many bad examples  the union of the prompts can cover.



% where $c$ is the number of bad examples whose probabilities are bigger than $t_r$





\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/squares.png}
    \caption{Test F1, coverage for different \ModelName subsets of different recalls. As we increase the recall of the subset, F1 first increases, and then decreases as the coverage goes down. If the coverage is not impacted, we can improve F1 by taking the subset of replies with higher recall. }
    \label{fig:coverage}
\end{figure}


==> useful_info <==
TAGS_TO_DETECT = (
    # good
    # "good",
    # "good/order_agreement",
    # "good/potential_bot_strategy",
    # bad_bot_strategy
    "bad_bot_strategy/information_leak",
    # game rule
    "game_rule/to_wrong_power",
    # description
    "description/wrong_justification",
    # timing
    "timing/missing_reply",
    "timing/late_reply",
    # order related
    "order/self/invalid",
    "order/others/invalid",
    "order/self/stupid_but_valid",
    "order/others/stupid_but_valid",
    "order/others/bad_for_self",
    # contradiction
    "contradiction/game_status",
    "contradiction/order_history",
    "contradiction/message_history",
    "contradiction/within_message",
    # "contradiction/pseudo_orders",
    # repetition
    "repetition/within_message",
    "repetition/between_message",
    # grammar
    "grammar",
    # other
    "other/general_nonsense",
    "other/weird_but_sensical",
    "other/wrong_term_used",
    "other/peculiar_stuff",
    # "other/should_not_appear/dead_power_talking",
    # "other/pscfr",
    # pseudo orders
    # "pseudoorders",
    # just bad
    "BAD_FAST",
)

# train/test distribution
WARNING:root:train_good: 4149
WARNING:root:train_bad: 561
WARNING:root:test_good: 1036
WARNING:root:test_bad: 139


# bad tag distribution
train: Counter({'BAD_FAST': 133, 'other/general_nonsense': 124, 'order/others/invalid': 48, 'grammar': 44, 'contradiction/game_status': 42, 'description/wrong_justification': 40, 'contradiction/within_message': 38, 'order/self/invalid': 33, 'contradiction/message_history': 32, 'order/others/stupid_but_valid': 21, 'repetition/between_message': 16, 'other/weird_but_sensical': 11, 'contradiction/order_history': 11, 'timing/late_reply': 9, 'order/self/stupid_but_valid': 7, 'other/wrong_term_used': 5, 'repetition/within_message': 4, 'game_rule/to_wrong_power': 4, 'other/peculiar_stuff': 3, 'bad_bot_strategy/information_leak': 3, 'order/others/bad_for_self': 2, 'timing/missing_reply': 1})

test: Counter({'BAD_FAST': 32, 'other/general_nonsense': 31, 'description/wrong_justification': 18, 'order/others/invalid': 16, 'contradiction/game_status': 14, 'grammar': 11, 'contradiction/within_message': 8, 'order/self/invalid': 8, 'order/others/stupid_but_valid': 7, 'contradiction/message_history': 7, 'repetition/between_message': 4, 'other/weird_but_sensical': 2, 'contradiction/order_history': 2, 'repetition/within_message': 1, 'timing/late_reply': 1, 'game_rule/to_wrong_power': 1})




# wrong justification examples
GERMANY -> ENGLAND(1613859788630235): i'm interested, but don't tell france that. i'll move my fleet to hel, so that i can take belgium and then start moving armies east
Comment: Moving to hel doesn't help with taking Belgium.



# other invalid example,

RUS->GER(1613860958720304): Are you moving in from Norway or the Barents Sea?
comment: Germany doesn\'t have a unit in Barents

# self invalid example

ENG->GER(1613860993735752): so. would you like support in to sweden from norway?
comment: England can\'t support this move.




# why weird prompts were generated when there are only 50 distractors

1. "thanks turkey" appears to be a "good" prompt because in the bad situations, many messages were sent to turkey; but in the distractor situations that survived top p, none of the messages were between turkey and other players (the model had to found situations where turkey appeared a lot in the state etc)

2. "works for me" appears because, the top bad situations were from the first sentences of S1901M where people propose things, but the phase distribution of the bad situations and distractors are really different, only 2 out 50 distractors are from S1901M, while 77 out of 550 in the bad situations are from S1901M

3. "where are you disband" also appears because in the bad situations, lots of messages were from the retreat phase, but retreat phases appear rarely in the distractors.
You sent November 29 at 11:19 PM
So I plan to sampling 500 distractors (maybe even more?), according to the (phase, turn in phase, player) distribution in the bad situations. But given that we have so many different situations, I am not sure if matching the (phase, turn in phase, player) distribution would be enough. If you have any thoughts on this, let me know. Basically we need really good distractors specific to different bad situations (e.g. order proposal, disband discussion, etc).
You sent November 29 at 11:20 PM
(i think turn in phase also matters because one phase can be really long, and "works for me" often appear when the context is short, even if we sample from S1901M, the context could still be super long, basically i think the context length also matters)
